Joint Spatio-Textual Reasoning for Answering Tourism Questions

Our goal is to answer real-world tourism questions that seek Points-of-Interest (POI) recommendations. Such questions express various kinds of spatial and non-spatial constraints, necessitating a combination of textual and spatial reasoning. In response, we develop the first joint spatio-textual reasoning model, which combines geo-spatial knowledge with information in textual corpora to answer questions. We first develop a modular spatial-reasoning network that uses geo-coordinates of location names mentioned in a question, and of candidate answer POIs, to reason over only spatial constraints. We then combine our spatial-reasoner with a textual reasoner in a joint model and present experiments on a real world POI recommendation task. We report substantial improvements over existing models with-out joint spatio-textual reasoning.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> conclusion.tex <==





\section{Conclusion} \label{sec:conclusion}
In this paper we presented a joint spatio-textual reasoning network, which combines a model designed for spatial (near/far) reasoning, with existing textual reasoning models. %We create and release a dataset of $9000$ question-answer pairs that require spatial reasoning. 
Experiments on an artificially constructed (spatial-only) QA dataset show that our spatial reasoner can effectively learn to satisfy spatial constraints. 
%We demonstrated how our spatial-reasoner is able to reason over location-mentions in questions, to return answers that satisfy subjective spatial constraints specified. %Further, the reasoner also learns to ignore location-mentions which serve as distractors and do not need to be considered for reasoning. 
We present detailed experiments highlighting the importance of our modeling choices. 

We also presented detailed experiments using our joint spatio-textual reasoning model on the recently released POI recommendation task that consists of real-world question-answers. We demonstrate our model improves state-of-the-art by 7\% (relative) on the full task and is also able to reason more effectively on spatial-questions as compared to baselines.

%Our work presents interesting directions for future work. As our error analysis shows XYZ.  Another interesting approach could be to extend ideas from existing Graph-neural network based approaches, such as NumNet \cite{NumNet}. Each entity could be viewed as a node in a graph for reasoning but we note that methods will need to be made more scalable for them to be useful. The entity space (and thus nodes in the graph) would run into thousands of nodes per question making current message passing based inference methods prohibitively expensive. 
%We will make the artificial dataset we generated as well as source code of our models available for research purposes. 

%TODO: TALK ABOUT A GRAPH NEURAL NETWORK APPROACH AND SCALABILITY CHALLENGE WITH NUMNET STYLE DENSE GRAPH 

==> introduction_OLD.tex <==
\section{Introduction} \label{sec:intro}
Recent work by \cite{TourQue} introduces the problem of answering tourism questions that seek Points-Of-Interest (POI) recommendations. 
%An interesting but understudied application of question answering relates to task of returning Points-Of-Interest (POI) recommendations to users based on their travel needs. 
%For example, consider the following question posted by a real user on a travel forum\footnote{shorturl.at/joDIM} about San Francisco: "\textit{Hi - I wonder if any locals can recommend good Italian and Californian restaurants in the Pacific Height neighborhood. Just looking for good food and ambience - not fine dining stuff! thanks}". Here the user is looking to have {\em good} "Italian and Californian" food in a specific neighbourhood of San Francisco ("Pacific Height") with budgetary constraints that indicate that they would not like expensive options. 
Figure \ref{fig:queryExample} shows an example of a real-world\footnote{http://shorturl.at/ablAK} POI-seeking question. Such questions tend to be noisy and long as users give more background about themselves and their needs. % in the question requiring models to resolve information need. 
In addition, the reasoning required for answering such questions is different from typical machine-reading comprehension \cite{squad,MultiRC2018,HOTPOTQA}, entailment-based reasoning or common-sense reasoning tasks \cite{BoolQ,CODAH,COSMOSQA,COMQA}. This is because, recommendations, by their very nature, are {\em subjective} and require models to reason over entity reviews that could also contain sarcasm, contradictions etc. %Reasoning over subjectivest constraints makes the reasoning task harder as there could be contradictory opinions expressed, sarcasm etc. 
Lastly, returning recommendations may also involve latent reasoning over symbolic information pertaining to the POI such as time, location, budgetary constraints, seating-capacity etc.  

\begin{figure}[]
 {\footnotesize
 %\begin{adjustwidth}{-2.2cm}{}
 %  Requires \usepackage{graphicx}
 \center
   \includegraphics[scale=0.51]{figs/LOC_question_example.jpg}
%   \vspace*{-3ex}
   \caption{\small Sample question from the dataset on Tourism Questions \cite{TourQue}. The answers correspond to POI IDs of the form $<$city\_id $>$\_$<$POI type$>$\_$<$number$>$. The dataset has three classes of POIs - restaurants (R), attractions (A) and hotels (H).}
   \label{fig:queryExample}
 %\end{adjustwidth}
 }
%\vspace*{-3ex}
 \end{figure}

While existing work on this task have attempted to address some of these challenges including question understanding \cite{MSEQ} as well as end-to-end answering using a collection of entity reviews \cite{TourQue}, the problem of jointly reasoning over symbolic knowledge such as, locations of entities, have not been explored. This is an important aspect because, as can be seen from the question in Figure \ref{fig:queryExample}, returning a restaurant recommendation that is close to the hotel mentioned in the question is important. %Thus, in order to make a useful recommendation, a model not only needs to suggest `good' restaurants they should also conform to locative constraints specified in the question. % spatial-reasoning  \cite{MSEQ,TourQue} on this problem has so far not addresses the need for {\em spatial-reasoning} while answering such questions. For instance, in Figure \ 

In this paper, we present our joint spatio-textual reasoning model for returning POI recommendations for users' questions. It uses a collection of POI reviews,  geographical co-ordinates of the POIs and location-mentions in the question, to jointly reason over entity reviews and their locations to make POI-recommendations. To the best of our knowledge, we are the first to develop such a model.% that is capable of jointly reasoning over subjective POI-review documents as well as distances between locations.  %Thus in the example above, an Italian or Californian restaurant recommendation that specifically does not fulfill the constraints of being in or close the Pacific Neighbourhood would be an incorrect recommendation. 
%We use the recently released data set\footnote{TODO:GitHub link to be inserted} on Tourism Questions \cite{TourQue} that consists of over 47,000 real-world POI question-answer pairs along with a universe of nearly 200,000 candidate POIs; questions are long and complex, as presented in Figure \ref{fig:queryExample}\footnote{ http://shorturl.at/fjkuv}, while the answers are represented by an ID corresponding to each POI. Each POI comes with a collection of reviews and meta-data that includes its geographical co-ordinates. %Figure \ref{fig:queryExample} presents an example\footnote{ http://shorturl.at/fjkuv} question-answer pair from this dataset. 
\subsection{Contribution}
We present a modular location reasoning network that can inject the ability to reason based on locations when combined with existing textual models ~\cite{TourQue} designed for the POI recommendations task. The network uses B-I-O markers for location-mentions in a question along with the vector representations of tokens; a combined question representation is then generated to determine {\em distance-weights} for each location token. These {distance-weights} are used with distances\footnote{distance from locations mentioned in the question} of candidate POIs, to return a location-based relevance score (Section \ref{sec:LRN}). In order to demonstrate the strength of our model, we create an artificial dataset that contains template-generated questions with simple location based constraints (Section \ref{sec:LRN}). We show that our locative reasoning network is not only able to reason over ``near'', ``'far'' constraints but is also able to determine locative references that are not useful for reasoning (Eg: a locative reference mentioning where a user last went on vacation). Finally, we present our joint model for spatio-textual reasoning (Section \ref{sec:joint}) that combines textual as well as locative reasoning for returning answers to real-world tourism questions. We demonstrate that our joint-model is able to perform better than models based only  location-reasoning or textual-reasoning. Our experiments indicate a XYZ\% improvement in location questions and an overall gain of ABC\% over existing models in the task of POI recommendations.[ TO BE FIXED]

%We demonstrate how we inject for details We present detailed experiments demonstrating how the locative reasoning network.  These We first demonstrate th [ADD 3-4 LINES OF DETAILS]. Our model results in x\% improvement on questions that have user location details or preferences specified in the question. 

% Our paper makes the following contributions:
% \begin{enumerate}
%     \item We present the novel task of answer POI recommendation questions incorporating locative constraints
%     \item We present our model that is capable of injecting the ability to reason over location data into existing architectures for POI recommendation.
%     \item We present detailed experiments demonstrating the strengths of our modeling choices. 
%     \item Toy dataset?
%     \item We show an X\% increase over ABC....
% \end{enumerate}
  
 
% We use a collection of question-answer pairs, entity reviews and g. We use the recently released dataset on Tourism Questions that contain over 47,000 question-answers pairs


%Despite the tremendous progress made by Question Answering systems over the last few years Geographical Information systems have seen limited gains in their ability to reason on geo-spatial data.  simple extracting reading comprehension tasks \cite{}, recent works have begun to show promising improvements in common-sense and multi-hop reasoning \cite{}, answering with knowledge bases and graphs \cite{} and more recently reasoning with numeric ability. 

==> model_joint_OLD.tex <==
%\section{Model} \label{sec:model}
\section{Spatio-Textual Reasoning Network}
\label{sec:joint}
The Spatio-Textual Reasoning Network (Figure \ref{fig:model}) consists of three components (i) Spatial Reasoner (ii) Textual Reasoner (iii) Joint Scoring Layer. 

We use SpNet as described in the previous section for spatial-reasoning and describe the rest of the components below: %describing some details about the textual-reasoning model used.

\noindent{\bf Textual-Reasoning sub-network:} We use the $\crq$ \cite{TourQue} model as our textual-reasoning sub-network. It consists of a Siamese-Encoder \cite{Siamese2} that uses question representations to attend over entity-review sentences and generate question-aware entity-embeddings. These entity embeddings are combined with question representations to generate an overall relevance score. For scalability, instead of using full review documents, the model uses a set of representative sentences from reviews after clustering them in USE-embedding space \cite{USE2018}. 
In order to build a model that is capable of joint spatio-textual reasoning, we learn question-specific combination weights that combine textual and spatial-reasoning scores.

\noindent{\bf Joint Scoring Layer:} Let the score generated by the textual-reasoner be $S_T$ and let the score generated by the spatial-reasoner be $S_L$. Let the rescaling weights for $S_T$ and $S_L$ be $w_T$ and $w_L$ respectively. 
Then, the overall score $S$ is given by: 
%\begin{equation*}
%    \alpha * sgm(WS_T)*tanh(W_lS_L) \\ + %\beta*sgm(W_tS_T)
%\end{equation*}
% \begin{equation*}
%   S=\alpha\sigma(w_TS_T)tanh(w_LS_L) + \beta\sigma(w_TS_T) %\beta*sgm(W_tS_T)
% \end{equation*}
$\alpha$*$\sigma(w_TS_T)*tanh(w_LS_L)$ + $\beta$*$\sigma(w_TS_T)$,  where $\sigma$ is the Sigmoid function and % $W_T,W_L$ are scaling weights learnt for $S_T$ and $S_L$ respectively. 
$\alpha$,$\beta$ are combination weights generated by a series of feedforward operations on the self-attended representation \cite{intra-attention} of the question (using a Question Encoder with the same architecture as in SpNet). %we use a self-attended  representation \cite{intra-attention} of its output states and down-project them after a series of feed-forward operations to generate two score combination weights ($\alpha$, $\beta$) %its output states are used to generate combination weights after a series of feed-forward operations over an attended representation of the output of the encoder 
%(See Figure \ref{fig:model}). %Let $q_a$ be the self-attended representation of the question. 
% \begin{equation*}
%     FF(x)= PReLU(W^{'}_lx+b^{'}_l)
% \end{equation*}
%where $W^{'}_l$, $b^{'}_l$ are the weight and bias terms learnt at each layer $l$. %Let $\alpha$, $\beta$ be the combination weights generated at the end of the FF(x) transformations, then %Each feed-forward operation applied
%Each feed-forward operation applies a PReLU~\cite{PRELU} activation on a linear layer. 
% The overall score $S$ is given by: 
% %\begin{equation*}
% %    \alpha * sgm(WS_T)*tanh(W_lS_L) \\ + %\beta*sgm(W_tS_T)
% %\end{equation*}
% $\alpha$ * $sgm(W_TS_T)*tanh(W_LS_L)$ + $\beta$*$sgm(W_TS_T)$, where $sgm$ is the Sigmoid function and $W_T,W_L$ are scaling weights learnt for $S_T$ and $S_L$ respectively. 
Note that, for questions where there are no locations mentioned, only textual-reasoning is required. It can be seen that in such cases the first term of the scoring equation acts as a {\em selector} where $S_L$ will be zero (distance vector $d_v$ will be a zero vector), thus letting the model rely only on textual-scores. 


%We use two textual models for POI recommendations [TO BE FIXED](i) $\cs$ \cite{TourQue} which is based on the Duet IR \cite{DUET2} model. The model compares elements of a question with different parts of a review document to  aggregate relevance for scoring. Local and distributed representations are used to capture lexical and semantic features. (ii) $\crq$ \cite{TourQue}, a model that uses a question representation to attend over a review sentences from a candidate to generate a relevance score. Instead of using full review documents, both models use a set of representative sentences from reviews after clustering sentences in USE-embedding space \cite{USE2018} for scalability \cite{TourQue}. We refer to spatio-textual models using $\cs$ and $\crq$ as $\csl$ and $\crlq$ respectively. Other recent textual models such as transformer-based MRC models do not scale for this dataset \cite{TourQue}.

\noindent{\bf Training: } We train the joint model using max-margin loss teaching the network to score the correct-answer higher than a negatively sampled candidate entity. Model parameters available in Suppl. Notes. 
\subsection{Evaluation}

We investigate the following research questions: (i) Does joint Spatio-Textual ranking result in improved performance over a model with only spatial-reasoning or only textual-reasoning? (ii)  How do pipelined baseline models that use spatial re-ranking perform on the task? (iii) Is the spatio-textual reasoning model more robust to distractor-locations as compared to baselines? (iv) What kind of errors does the model make? 

%\subsubsection{Dataset}
\noindent{\bf Dataset:}
We use the recently released data set\footnote{https://github.com/dair-iitd/TourismQA} on Tourism Questions \cite{TourQue} that consists of over 47,000 real-world POI question-answer pairs along with a universe of nearly 200,000 candidate POIs; questions are long and complex, as presented in Figure \ref{fig:queryExample}, while the recommendations (answers) are represented by an ID corresponding to each POI. Each POI comes with a collection of reviews and meta-data that includes its geo-coordinates. The training set contains nearly $38000$ QA-pairs and about $4200$ QA-pairs each in  the validation and test sets. The average candidate space for each question is $5300$. % and testing.

{\noindent \bf Task Challenges: } The task presents novel challenges of reasoning and scale; the nature of entity reviews (eg. inference on subjective language, sarcasm etc) makes methods such as BM25 \cite{BM25}, that are often used to prune the search space quickly in large scale QA tasks \cite{drqa,SearchQA}, ineffective. %The textual reasoning required for answering questions in this dataset is different from typical machine-reading comprehension \cite{MultiRC2018,HOTPOTQA}, entailment-based reasoning or common-sense reasoning tasks \cite{BoolQ,COSMOSQA,COMQA}. This is because, recommendations, by their very nature, are {\em subjective} and require models to reason over entity reviews that could also contain sarcasm, contradictions etc. In addition, the large answer space and the need to reason over thousands of review documents makes this dataset even more challenging. 
Thus, even simple BERT-based architectures or popular models such as BiDAF \cite{BIDAF} do not scale for the answering task in this dataset \cite{TourQue}. Thus, we use the non-BERT based SpNet subnetwork in the rest of the QA experiments. %We therefore, do not use BERT SpNet for experiments on this task.

\noindent{\bf Location Tagging: }
In order to get mentions of locations in questions, we manually label a set of $425$ questions from the training set for location mentions. We then use a BERT-BiLSTM CRF \cite{MSEQ} based tagger trained on this set to label locations.  The tagger has a macro-$F1$ of 88.03. The tagger tags all location mentions in a question without considering its utility for spatial-reasoning. Since this a real-world dataset, it is possible that a question may contain {\bf only} distractor-locations, i.e., locations-mentions that do not need to be reasoned over the answering task. %Table \ref{tab:location-tagger-results} shows the accuracy of the tagger on a small devset of $75$ questions. 
% \begin{table}[ht]
% \scriptsize
% \centering
% \begin{tabular}{|l|l|l|l|}
% \hline
%  & \textbf{Precision} & \textbf{Recall} & \textbf{F1} \\ \hline
% \textbf{Micro Average} & 87.59 & 87.56 & 87.58 \\ \hline
% \textbf{Macro Average} & 88.24 & 87.83 & 88.03 \\ \hline
% \end{tabular}%
% \caption{Performance of the BERT-BiLSTM CRF for tagging locations.}
% \label{tab:location-tagger-results}
% \end{table}
% \begin{table}[H]
% \scriptsize
% \centering
% \begin{tabular}{|l|l|l|l|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{\textbf{}} & \multicolumn{2}{c|}{\textbf{Location}} & \multicolumn{2}{c|}{\textbf{Non-location}} \\ \hline
% \multicolumn{1}{|c|}{\textbf{Dataset}} & \multicolumn{1}{c|}{\textbf{Questions}} & \multicolumn{1}{c|}{\textbf{QA pairs}} & \multicolumn{1}{c|}{\textbf{Questions}} & \multicolumn{1}{c|}{\textbf{QA pairs}} \\ \hline
% Train & 9,617 & 21,396 & 10,342 & 22,150 \\ \hline
% Dev & 1,065 & 2,209 & 1,054 & 1,987 \\ \hline
% Test & 1,086 & 2,198 & 1,087 & 2,144 \\ \hline
% \end{tabular}
% \caption{Distribution of questions with location-mention across train, dev \& test sets.}
% \label{tab:loc-stats-table}
% \end{table}

We label all questions in the full dataset using this tagger, resulting in approximately 49.54\% of the QA pairs containing at least one location-mention (See suppl. notes). %Table \ref{tab:loc-stats-table}). %21396, 2209 and 2198 QA pairs with location-mentions in the training, validation and test-dataset respectively.
We use the Bing Maps Location API\footnote{https://docs.microsoft.com/en-us/bingmaps/rest-services/locations/} to geo-tag all location mentions.
\begin{table}
\scriptsize
\center
\begin{tabular}{|c|l|l|l|l|l|}
\hline
\multicolumn{1}{|l|}{}                                          & \multicolumn{5}{|c|}{Location Questions}                                \\ \hline
\multicolumn{1}{|c|}{\bf Models}                                          & \textbf{Acc@3} & \textbf{Acc@5} & {\bf Acc@30} & \textbf{MRR} & $\mathbf{Dist_g}$ \\\hline
SD                                                            &           2.49    &       3.41       &  14.29   &    0.029     &       3.07      \\ \hline
SpNet   &    1.47    &                                                21.12            &       8.47              & 0.019   &       2.97          \\ \hline \hline
%$\cs$                                                          &      15.84          &     20.26        &  51.47    &   0.149    &      2.61      \\ \hline
%$\cs$ $\rightarrow$ SD        &   11.34             &   17.26     &   51.47     &      0.118        & 2.18             \\ \hline
%$\cs$ $\rightarrow$ LocNet     &      8.38          &  13.72     &  51.47       & 0.097                &    2.27         \\ \hline
%\begin{tabular}[c]{@{}c@{}}Spatio-textual\\ $\cs$\end{tabular} &                &           &     &              &             \\ \hline \hline
CRQA                                                          &       14.83         &       21.27        &  50.65   &   0.143      &    3.41         \\ \hline
CRQA$\rightarrow$SD       &      13.73          &   19.26   &   50.65       &   0.125           &       {\bf 2.23}      \\ \hline
CRQA$\rightarrow$SpNet     & 10.13               &  15.65   &    50.64       &  0.104            &     2.47        \\ \hline
\begin{tabular}[c]{@{}c@{}}Spatio-textual\\ CRQA\end{tabular} &    {\bf 18.32}        &       {\bf 25.69} &     {\bf 56.17}     &      {\bf 0.168}        &      2.62         \\ \hline
\end{tabular}
\caption{Comparison of the joint Spatio-Textual model with baselines on questions that have location mentions} 
\label{tab:main-loc-results}
\end{table}
\subsubsection{Baselines}
%\noindent{\bf Baselines:}
Apart from the textual-reasoning model $\crq$ we also use the following baselines in our experiments:

\noindent{\bf Sort-by-distance (SD)}: Given a set of tagged-locations in a question and their geo-coordinates, rank candidate entities by the {\em minimum} distance from the set of tagged locations.

\noindent{\bf SpNet}: Use only the spatial-reasoning network for ranking candidate entities using their geo-coordinates. No textual-reasoning performed.

\noindent{\bf $\crq$ $\rightarrow$ SD:} Rank candidates using $\crq$ and then re-rank the top-30 answers using SD.

\noindent{\bf $\crq$ $\rightarrow$ SpNet:} Rank candidates using $\crq$ and then re-rank the top-30 answers using SpNet.



\begin{table*}
\scriptsize
\begin{tabular}{|c|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multicolumn{1}{|l}{} & \multicolumn{5}{|c}{Location Questions} & \multicolumn{4}{|c}{Non-location Questions} & \multicolumn{4}{|c|}{Full Set} \\ \cline{2-14}
\multicolumn{1}{|c|}{Models} & \textbf{Acc@3} & \textbf{Acc@5} & \textbf{Acc@30} & \textbf{MRR} & \textbf{$Dist_g$} & \textbf{Acc@3} & \textbf{Acc@5} & \textbf{Acc@30} & \textbf{MRR} & \textbf{Acc@3} & \textbf{Acc@5} & \textbf{Acc@30} & \textbf{MRR} \\ \hline
%SD                                                            &                &                &              &              &                               - &              - &           -  &             -   &            -    &  -            \\ \hline
%LocNet                                                        &                &                &              &             &                              -  &  -             &     -        &       -         &           -     &             - \\ \hline \hline
%$\cs$                                                          & 15.84          &     20.26        &    0.149    &      2.61 &          18.68    &      25.94         &  0.174      &    17.26  &            23.10    &               0.161              \\ \hline
%$\cs$+SD        &                &                &              &             &                               - &        -      &         -    &               - &                - &       -       \\ \hline
%$\cs$+LocNet     &                &                &              &             &                               &              &             &                &                &              \\ \hline
%\begin{tabular}[c]{@{}c@{}}Spatio-Textual\\ $\cs$\end{tabular} &                                &              &             &                &                &              &             &                &                &        \\ \hline \hline
CRQA & 14.83 & 21.27 & 50.65 & 0.143 & 3.41 & 18.95 & 26.22 & 54.37 & 0.177 & 16.89 & 23.75 & 52.51 & 0.159 \\ \hline
%CRQA+SD       &                               &              &             &                &                &              &             &                &                &              \\ \hline
%CRQA+LocNET     &                                &              &             &                &                &              &             &                &                &              \\ \hline
\begin{tabular}[c]{@{}c@{}}Spatio-Textual\\ CRQA\end{tabular} 
& {\bf 18.32} & {\bf 25.69} & {\bf 56.17} & {\bf 0.168} & {\bf 2.62 }& {\bf 20.42} & {\bf 26.77} & {\bf 56.49} & {\bf 0.18 }& {\bf 19.37} & {\bf 26.23} & {\bf 56.33} & {\bf 0.175} \\
  
\hline
\end{tabular}
\caption{Comparison of the joint Spatio-Textual model with its textual model counterpart} 
\label{tab:main-results}
%\vspace{-1ex}
\end{table*}


\noindent{\bf Training:} We first pretrain SpNet on this dataset by allowing entities within a radius of $100$m from the actual gold-entity to be considered as gold. In order to train the joint network we initialize model parameters learnt from component-wise pretraining of both SpNet as well as $\crq$. Please see suppl. notes for details about hyper-parameter settings.

\subsubsection{Results} \label{sec:results-main}
%\noindent{\bf Spatio-Textual Reasoning:}
We present our experiments on two slices of the test-set -- questions with tagged location-mentions (called {\em Location-Questions}) and those without any location mentions ({\em Non-Location Questions}). As can be seen in Table \ref{tab:main-loc-results} sorting-by-distance (SD) performs very poorly indicating that simple methods for ranking based on entity-distance do not work for such questions. Further, the poor performance of the spatial-reasoning network (SpNet) also indicates that the task cannot be solved just by reasoning on location data. 

In addition, pipelined re-ranking using SD or SpNet over the textual reasoning model decreases the average distance ($Dist_g$) from the gold-entity but does not result in improved performance in terms of answering (Acc@N) indicating the need for spatio-textual reasoning. Finally, from Tables \ref{tab:main-loc-results} \& \ref{tab:main-results} we note that the spatio-textual model performs better than its textual counterpart on the Location-Questions subset, while continuing to perform well on questions without location mentions. 


\noindent{\bf Effect of distractor-locations:}
As mentioned earlier, we use a location-tagger that is oblivious to the reasoning task, to tag locations in the dataset. This could result in questions that only contain distractor-locations but are considered as a spatial-question while reasoning. To study this, we manually create a small set of $200$ questions, randomly selected from the test-set, but ensuring that half of it contains {\em at least} one non-distractor location mentioned in the question while the other half contains questions with {\em only} distractor-locations. % (i.e, none of the tagged locations are required for spatial-reasoning).%  Table \ref{tab:main-clean-results} reports results on this small set of location-questions.

% \begin{table*}[ht]
% \scriptsize
% \center
% \begin{tabular}{|c|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \multicolumn{1}{|l|}{} & \multicolumn{5}{|c}{Questions requiring Spatial-reasoning} & \multicolumn{5}{|c|}{Questions with distractor-locations only} \\ \hline
% \multicolumn{1}{|c|}{\bf Models} & \textbf{Acc@3} & \textbf{Acc@5} & \textbf{Acc@30} & \textbf{MRR} & \textbf{Dg} & \textbf{Acc@3} & \textbf{Acc@5} & \textbf{Acc@30} & \textbf{MRR} & \textbf{Dg} \\\hline
% SD & 5.00 & 7.00 & 22.00 & 0.053 & 2.10 & 2.00 & 3.00 & 17.00 & 0.025 & 4.12 \\ \hline
% SpNet & 1.00 & 1.00 & 8.00 & 0.013 & 2.64 & 1.00 & 2.00 & 9.00 & 0.016 & 4.14 \\ \hline \hline
% %$\cs$ & 13.00 & 16.00 & 45.00 & 0.128 & 2.30 \\ \hline
% %$\cs$ $\rightarrow$ SD & 14.00 & 20.00 & 45.00 & 0.110 & 1.75 \\ \hline
% %$\cs$ $\rightarrow$ LocNet & 9.00 & 14.00 & 45.00 & 0.092 & 2.11 \\ \hline
% %\begin{tabular}[c]{@{}c@{}}Spatio-textual\\ $\cs$\end{tabular} 
% %&  &  &  &  &  \\ \hline \hline
% CRQA & 15.00 & 17.00 & 51.00 & 0.132 & 3.53 & 19.00 & 26.00 & 51.00 & 0.162 & 3.62 \\ \hline
% CRQA$\rightarrow$SD & 15.00 & 22.00 & 51.00 & 0.142 & {\bf 1.96} & 13.00 & 17.00 & 51.00 & 0.108 & 3.26 \\ \hline
% CRQA$\rightarrow$SpNet & 16.00 & 23.00 & 51.00 & 0.134 & 2.41 & 13.00 & 17.00 & 51.00 & 0.113 & {\bf 3.24} \\ \hline
% \begin{tabular}[c]{@{}c@{}}Spatio-textual\\ CRQA \end{tabular}
% & {\bf 22.00} & {\bf 28.00} & {\bf 54.00} & {\bf 0.182} & 2.62 & {\bf 20.00} & {\bf 28.00} & {\bf 53.00} & {\bf 0.187} & 3.50 \\ \hline
% \end{tabular}
% \caption{Comparison of the joint Spatio-Textual models with baselines on two subsets from the test-set: (i) Questions requiring Spatial-reasoning (ii) Questions with distractor-locations only (no spatial reasoning required)} 
% \label{tab:main-loc-clean-results}
% \end{table*}


As can be seen from Table \ref{tab:main-loc-clean-results}, %$\crq$ is almost unaffected by location distractors as it does not reason over spatial data. However, 
all models including the spatio-textual model deteriorate in performance if a question only contains distractors; the spatio-textual model however, suffers a less significant drop in performance. %are affected by the presence of distractor-locations especially if a question only contains distractor-location. %However, models based on SD or SpNet re-ranking %Further, experiments on the set of questions with only distractor-locations shows a significant drop in performance of baseline methods while the spatio-textual reasoner is able to recognize that the location-mentions are unhelpful.

\begin{table}
\scriptsize
\center
\begin{tabular}{|c|l|l|l|l|l|}
\hline
\multicolumn{1}{|l|}{}                                          & \multicolumn{5}{|c|}{Questions requiring Spatial-reasoning}                                \\ \hline
\multicolumn{1}{|c|}{\bf Models}                                          & \textbf{Acc@3} & \textbf{Acc@5} & {\bf Acc@30} & \textbf{MRR} & \textbf{$Dist_g$} \\\hline
SD                                                            &           5.00    &       7.00      &  22.00   &    0.053     &       2.10      \\ \hline
SpNet   &    1.00    &                                                1.00           &       8.00            & 0.013   &       2.64          \\ \hline \hline
CRQA                                                          &       15.00         &       17.00        &  51.00   &   0.132      &    3.53         \\ \hline
CRQA$\rightarrow$SD       &      15.00          &   22.00   &   51.00       &   0.142           &       {\bf 1.963}      \\ \hline
CRQA$\rightarrow$SpNet     & 16.00               &  23.00   &    51.00       &  0.134            &     2.41        \\ \hline
\begin{tabular}[c]{@{}c@{}}Spatio-textual\\ CRQA\end{tabular} &    {\bf 22.00}        &       {\bf 28.00} &     {\bf 54.00}     &      {\bf 0.182}        &      2.62         \\ \hline
\multicolumn{1}{|l|}{}                                          & \multicolumn{5}{|c|}{{Questions with distractor-locations only}}                                \\ \hline
SD                                                            &           2.00    &       3.00       &  17.00   &    0.025     &       4.12      \\ \hline
SpNet   &    1.00    &                                                2.00           &       9.00              & 0.016   &       4.14          \\ \hline \hline
CRQA                                                          &       19.00         &       26.00        &  51.00   &   0.162      &    3.62         \\ \hline
CRQA$\rightarrow$SD       &      13.00          &   17.00  &  51.005       &   0.108          &       { 3.26}      \\ \hline
CRQA$\rightarrow$SpNet     & 13.00               &  17.00   &    51.00       &  0.113            &     {\bf 3.24}        \\  \hline
\begin{tabular}[c]{@{}c@{}}Spatio-textual\\ CRQA\end{tabular} &    {\bf 20.00}        &       {\bf 28.00} &     {\bf 53.00}     &      {\bf 0.187}        &      3.50         \\ \hline
\end{tabular}
\caption{%Comparison of the joint Spatio-Textual models with baselines 
Experiments on two subsets from the test-set: (i) Questions requiring Spatial-reasoning (ii) Questions with distractor-locations only.}% (no spatial reasoning required)} 
\label{tab:main-loc-clean-results}
%\vspace{-3ex}
\end{table}
%\subsection{}

%\subsubsection{Qualitative Study}
\noindent{\bf Qualitative Study:}
We randomly selected $150$ QA pairs with location-mentions from the test-set, to conduct a qualitative error analysis of Spatio-textual $\crq$. We find that approximately 37\% of the errors can be traced to the textual-reasoner, 22\% of the errors were due to a `near' constraint not being satisfied, while approximately 13\%  of the errors were due to the model reasoning on distractor-locations. Further, another 8\% of the errors were due to errors made by the location-tagger and incorrect geo-spatial data (See Suppl. notes for details). 
%1. Some will be "staying at X, but want close to city center" -- we wont get for city center
%TO BE ADDED


%\subsubsection{Effect of Search Space}
\noindent{\bf Effect of Candidate Search Space:}
\begin{table}
\scriptsize
\center
\begin{tabular}{|c|l|l|l|l|l|}
\hline
\multicolumn{1}{|l|}{}                                          & \multicolumn{5}{|c|}{Location Questions}                                \\ \hline
\multicolumn{1}{|c|}{\bf Models}                                          & \textbf{Acc@3} & \textbf{Acc@5} & {\bf Acc@30} & \textbf{MRR} & \textbf{$Dist_g$} \\\hline
%SD                                                            &           2.49    &       3.41       &  14.29   &    0.029     &       3.07      \\ \hline
%LocNet                                                        &                &                &      &        &             \\ \hline \hline
%$\cs$                                                          &      15.84          &     20.26        &  {\bf 51.47}    &   0.149    &      2.61      \\ \hline
%$\cs$ $\rightarrow$ SD        &   11.34             &   17.26     &   {\bf 51.47}     &      0.118        & {\bf 2.18}             \\ \hline
%$\cs$ $\rightarrow$ LocNet     &      8.38          &  13.72     &  {\bf 51.47}       & 0.097                &    2.27         \\ \hline 
$\csr$ & 19.89 & 26.43 & {\bf 51.47} & 0.168 & 2.70 \\ \hline
\begin{tabular}[c]{@{}c@{}}Spatio-textual\\ CSRQA\end{tabular} 
& {\bf 21.36} & {\bf 28.36} & {\bf 51.47} & {\bf 0.183} & 2.27 \\ \hline
\multicolumn{1}{|l|}{}                                          & \multicolumn{5}{|c|}{All Questions}                                \\ \hline
%\multicolumn{1}{|c|}{\bf Models}                                          & \textbf{Acc@3} & \textbf{Acc@5} & {\bf Acc@30} & \textbf{MRR} & \textbf{Dg} \\\hline
%SD                                                            &           2.49    &       3.41       &  14.29   &    0.029     &       3.07      \\ \hline
%LocNet                                                        &                &                &      &        &             \\ \hline \hline
%$\cs$                                                          &      15.84          &     20.26        &  51.47    &   0.149    &      2.61      \\ \hline
%$\cs$ $\rightarrow$ SD        &   11.34             &   17.26     &   51.47     &      0.118        & 2.18             \\ \hline
%$\cs$ $\rightarrow$ LocNet     &      8.38          &  13.72     &  51.47       & 0.097                &    2.27         \\ \hline \hline

$\csr$ & 21.45 & 28.21 & {\bf 52.65} & 0.186 & 2.47 \\ \hline
\begin{tabular}[c]{@{}c@{}}Spatio-textual\\ CSRQA\end{tabular} 
& {\bf 22.41} & {\bf 28.99} & {\bf 52.65} & {\bf 0.193} & {\bf 2.32}\\ \hline

\end{tabular}


\caption{Comparison with current state-of-the-art $\csr$ on (i) Location Questions (ii) Full Task} %The $\csr$ model is a $\cs$ $\rightarrow$ $\crq$ model and the 
%Spatio-textual $\csr$ refers to re-ranking using the spatio-textual $\crq$ instead of $\crq$.} % joint Spatio-Textual models with pipe-lined baselines using SD (Sort-by-distance) and Location Reasoning (LocNET) on questions that have location mentions} 
\label{tab:csr-loc-results}
\end{table}
Similar to \citet{TourQue} we also experiment on this dataset by employing a neural method to reduce the search space \cite{DUET2} before using the $\crq$ textual-reasoner to re-rank only the top-30 selected candidates (pipeline referred to as $\csr$).
%Similar to other large scale QA tasks \cite{AMANDATriviaQA}, this task also has a very large search space and \citet{TourQue}. %However, BM25 \cite{BM25} a commonly used method to reduce search space in QA tasks \cite{drqa}, does not work on this task due to the nature of entity-review documents \cite{TourQue}. To help reduce the search space before ranking candidates, the \citet{TourQue} 
%use a fast and scalable neural-IR method based on Duet \cite{DUET2} (referred to as $\cs$ in their work) to to filter candidates and reduce the search space. They then use $\crq$ to re-rank candidates to return answers. Unlike $\crq$, which uses two levels of attention between question and review sentences to score candidate entities $\cs$ does not reason deeply over the text.%. It compares elements of a question with different parts of a review document to aggregate relevance for scoring. Local and distributed representations are used to capture lexical and semantic features. The model thus, 
%that does not deeply reason over text unlike $\crq$, which uses two levels of attention between question and review sentences to score candidate entities. Thus, \citet{TourQue} propose the $\csr$ model which first uses $\cs$ to filter candidates and reduce the search space, and then uses $\crq$ to re-rank candidates to return answers.
%The $\csr$ model consists of a selector followed by the use of the textual reasoner $\crq$. 
We thus, replace the $\crq$ model with its spatio-textual equivalent in $\csr$ and refer to it as Spatio-Textual $\csr$.  We report the results of this experiment in Table \ref{tab:csr-loc-results} and find that it results in a 1 pt (Acc@3) improvement overall, and a 1.5 pt improvement on location questions (Acc@3), establishing new state-of-the-art results. We note that because the selector is incapable of spatial-reasoning it possibly reduces the gains made by the spatio-textual ranking. An interesting direction of future work could thus, be to augment general purpose neural-IR methods with such spatial-reasoning. 

%We conduct a blind-human study on the results of both $\csr$ and spatio-textual $\csr$ and find that our model continues to outperform the baseline % in generic neural-IR methods.  %, but it still results in a 1pt (Acc@3) improvement overall, and a 1.5pt improvement on location questions (Acc@3). % the As compared to the current state-of-the-art $\csr$ model, we report a $7$\% relative improvement on location questions and a $4.5\%$ relative improvement on the overall task, using this model.






% \begin{table}[ht]
% \scriptsize
% \center
% \begin{tabular}{|c|l|l|l|l|l|}
% \hline
% \multicolumn{1}{|l|}{}                                          & \multicolumn{5}{|c|}{All Questions}                                \\ \hline
% \multicolumn{1}{|c|}{\bf Models}                                          & \textbf{Acc@3} & \textbf{Acc@5} & {\bf Acc@30} & \textbf{MRR} & \textbf{Dg} \\\hline
% %SD                                                            &           2.49    &       3.41       &  14.29   &    0.029     &       3.07      \\ \hline
% %LocNet                                                        &                &                &      &        &             \\ \hline \hline
% %$\cs$                                                          &      15.84          &     20.26        &  51.47    &   0.149    &      2.61      \\ \hline
% %$\cs$ $\rightarrow$ SD        &   11.34             &   17.26     &   51.47     &      0.118        & 2.18             \\ \hline
% %$\cs$ $\rightarrow$ LocNet     &      8.38          &  13.72     &  51.47       & 0.097                &    2.27         \\ \hline \hline

% $\csr$ & 21.45 & 28.21 & {\bf 52.65} & 0.186 & 2.47 \\ \hline
% \begin{tabular}[c]{@{}c@{}}Spatio-textual\\ CSRQA\end{tabular} 
% & {\bf 22.41} & {\bf 28.99} & {\bf 52.65} & {\bf 0.193} & {\bf 2.32}\\ \hline
% \end{tabular}
% \caption{Comparison with current state-of-the-art $\csr$ on the full task.} % joint Spatio-Textual models with pipe-lined baselines using SD (Sort-by-distance) and Location Reasoning (LocNET) on questions that have location mentions} 
% \label{tab:csr-loc-results}
% \end{table}
%On the subset of the test data that contains only As can be seen in table \ref{tab:main-loc-results}

%Baselines: (1) CS (2) CR (3) LocNet (radius as gold) (4) LocNet (full task) (5) Rank with CS, sort by LocNet (6) Rank with LocNet, Sort by CS (7) Rank with CS, sort by distance (8) Rank by distance, sort with CS -- REPEAT FOR CR. (9), (10), (11), (12). Metrics: Acc@3,Acc@5,MRR, $D_g$.

%+ 

%CSR based [ looks out of place but can add.]
%The Location Reasoning network generates a pluggable score 

%The tagging of locations mentioned in the question for the real data is discussed in a separate section.

% This consists of series of stacked blocks. Each block consists of a Linear layer with ReLU \cite{Relu} activation. - uses the encoded question representation and generates weights for each token position indicating its importance for distance-based scoring. The MLP returns a value for each state of the GRU representation. 

